Contracting edges to destroy a pattern: A complexity study

Given a graph G and an integer k, the objective of the $\Pi$-Contraction problem is to check whether there exists at most k edges in G such that contracting them in G results in a graph satisfying the property $\Pi$. We investigate the problem where $\Pi$ is `H-free' (without any induced copies of H). It is trivial that H-free Contraction is polynomial-time solvable if H is a complete graph of at most two vertices. We prove that, in all other cases, the problem is NP-complete. We then investigate the fixed-parameter tractability of these problems. We prove that whenever H is a tree, except for seven trees, H-free Contraction is W[2]-hard. This result along with the known results leaves behind three unknown cases among trees.

==> algorithms/tk1.tex <==
\subsection{Contraction to $tK_1$-free graphs}
In this section, we assume that $t\geq 2$.

\begin{mdframed}
  \textbf{\TKVD}\\ 
  Given a graph $G$ and an integer $k$, can $G$ be modified into a $tK_1$-free graph by deleting at most $k$ vertices?\\
  \textbf{Parameter}: $k$
\end{mdframed}

There is a simple bounded search tree algorithm given in \cite{DBLP:journals/ipl/Cai96} to solve \TKVD\ in FPT time. 
The algorithm gives a set $V_k$ of vertices of the input graph $G$ such that $|V_k|\leq k$ and $G - V_k$ is $tK_1$-free, if such a set $V_k$ exists. We use this algorithm in the Step 1 of the following algorithm for \TKC.\\

\noindent
\textbf{Algorithm for }\TKC\\
\noindent
\textbf{Input:} A graph $G$ and an integer $k$
\begin{description}
    \item[Step 1:] 
    Run the algorithm for \TKVD\ with input $(G, 2k)$. If it obtains ``No'' then return ``No''. If it returns a set $V_k$
    of at most $2k$ vertices such that $G - V_k$ is $tK_1$-free, then let $V_c = V(G)\setminus V_k$.
    \item[Step 2:] For each possible set $S_0$ of at most $k$ contractions in $G[V_k]$, do the following:
    \begin{myEnumerate}
        \item Let $G_1 = G/S_0$, $k_1 = k-|S_0|$, and $V'_{k} = V(G_1)\setminus V_c$.
        \item For every possible partition $(R, R_0)$ of $V'_{k}$ such that every vertex in $R$ has at least one neighbor in $V_c$, do the following:
        \begin{myEnumerate}
            \item For each $1\leq i\leq t-1$, do the following:
            \begin{myEnumerate}
                \item Initialize $T_i = \emptyset$.
                \item Let $T' = \bigcup_{j=1}^{j=i-1}T_j$.
                \item For every nonnegative integer partition $(\ell_0,\ell_1,\ell_{2})$ of $t$, do the following:
                For every set $L_0\in 2^{R_0}$ and $L_1\in 2^{T'}$ 
                such that $|L_0|=\ell_0$ and $|L_1|=\ell_1$, let $Z_{L_0, L_1}$
                be a maximal set of disjoint sets $L_2\subseteq V_c\setminus T'$ such that $|L_2|=\ell_2$ and
                $L_2$ is an independent set and there is no edge between $L_2$ and $L_0\cup L_1$.
                Arbitrarily choose $\min\{k+1, |Z_{L_0, L_1}|\}$ sets from
                $Z_{L_0, L_1}$ and add the vertices in the chosen sets into $T_i$.
            \end{myEnumerate}
            \item Let $T= \bigcup_{i=1}^{i=t-1}T_i$.
            \item For every partition $(R_1,R_2)$ of $R$ such that every vertex in $R_1$ has at least one neighbor in $T$, do the following:
            \begin{myEnumerate}
                \item For each possible set $S_1$ of at most $k_1$ contractions in $G_1[R_1,T]$ such that every vertex in $R_1$ is an end vertex
            of some edge in $S_1$, do the following:
                \begin{myEnumerate}
                    \item Let $G_2 = G_1/S_1$, $k_2 = k_1 - |S_1|$.
                    \item For every vertex $u_i$ in $R_2$, arbitrarily choose a neighbor $v_i$ of $u_i$ in $V_c\setminus T$. 
                    Let $S_2$ be the set of all such $u_iv_i$ edges. Let $G_3 = G_2/S_2, k_3 = k_2 - |S_2|$.
                    \item For every vertex $u_i\in V_c\setminus T$, arbitrarily choose a neighbor $v_i$ (if exists) of $u_i$ in 
                    $V_c\setminus T$. Let $P$ be the set of all such $v_i$s.
                    \item For every possible set $S_3$ of at most $k_3$ contractions in $G_3[T\cup P]$, do the following.
                    \begin{myEnumerate}
                        \item $G_4 = G_3/S_3, k_4 = k_3 - |S_3|$.
                        \item If $k_4 \geq 0$ and $G_4$ is $tK_1$-free, then return ``YES''.
                    \end{myEnumerate}
                \end{myEnumerate}
            \end{myEnumerate}
        \end{myEnumerate}
    \end{myEnumerate}
    \item[Step 3:] Return ``NO''
\end{description}

\begin{lemma}
\label{lem:tk1}
Let $(G,k)$ be a yes-instance of \TKC.
Then the algorithm returns ``YES''.
\end{lemma}
\begin{proof}
Let $S^*$ be a solution of $(G,k)$. We will show that there exists a set $S = S_0\cup S_1\cup S_2\cup S_3$ 
of at most $k$ contractions such 
that $G/S$ is $tK_1$-free and this is obtained in one branch of the algorithm. 
Consider the branch such that $S_0 = S^*\cap E[V_k]$. 
Let $V'_{k}$ be the resultant set of vertices of $V_k$. 
Let $R_0$ be the set of vertices in $V'_{k}$ which are not touched by 
$S^*\setminus S_0$ and let $R= V'_{k}\setminus R_0$. 
Let $T_i$ for $1\leq i\leq t-1$ and $T$ be as defined in the algorithm. 
Let $R_1$ be the end vertices in $R$ of edges in $S^*\cap E[R,T]$, and let $R_2= R\setminus R_1$. 
Consider the sub-branch such that $S_1 = S^*\cap E[R_1,T]$
and let $S_2$ be as obtained in the algorithm in this branch. 
Let $S'_3 = S^*\cap E[T]$. For every edge $uv$ in $S^*$ such that $u\in T$ 
and $v\in V_c\setminus T$, consider an edge $uu_p$, where $u_p$ is an arbitrary neighbor of $u$ in $P$. Let such edges $uu_p$ form the set $S''_3$.
Consider the branch in which $S_3 = S'_3\cup S''_3$.
We will prove that $S = S_0\cup S_1\cup S_2\cup S_3$ is a solution. 

Clearly, $|S|\leq k$ as $|S^*|\leq k$. 
For a contradiction, assume that $G/S$ has a $tK_1$ formed by $U=\{u_1,u_2,\ldots,u_t\}$. 
Let $M_i$ be the subset of vertices in $G$ corresponding to $u_i$, i.e., $M_i$ induces a connected subgraph of $G$ such that it is 
contracted to a single vertex $u_i$ in $G/S$. 
Let $\mathcal{M}=\{M_i | 1\leq i\leq t\}$.
Let $T_0 = R_0$ and $T_t = V_c\setminus T$. 
Let $ind(M_i)$ be the largest integer $j$ such that $M_i\cap T_j\neq \emptyset$.
Let $I = \{ind(M_i) | 1\leq i\leq t\}$. Since $|I|\leq t$, and there are $t+1$ potential indices ($0,1,\ldots,t$), 
there is at least one index $j$ (for $0\leq j\leq t$) not in $I$. Clearly, $j\neq 0$, as otherwise $V_c$ is not $tK_1$-free.
Assume that $t \notin I$. Then, since every contraction in $S^*$ in $E[T]$ is also in $S$, $U$ forms a $tK_1$ in $G/S^*$, 
which is a contradiction. Therefore, $t\in I$.
Then $1\leq j\leq t-1$. Let $\mathcal{M}'$ be the subset of $\mathcal{M}$ where each set in $\mathcal{M}'$ is a subset of $\bigcup_{i=0}^{i=j-1}T_j$.
Then by the construction, $T_j$ has a set $\mathcal{J}$ of $k+1$ independent sets $J$ of size $t-|\mathcal{M}'|$ 
(otherwise, every vertex in the sets in $\mathcal{M}\setminus M'$ would have been in $T_j$) 
such that every vertex in $J$ is nonadjacent to each set in $\mathcal{M}'$. This implies that each such set $J$ is affected by a contraction (which does not affect other sets in $\mathcal{J}$) in $S^*$. This implies that $|S^*|>k$, a contradiction.
\end{proof}

Now, Theorem~\ref{thm:tk1} follows from Lemma~\ref{lem:tk1} and from 
the fact that the algorithm returns ``YES'' only when it finds a solution of size at most $k$.
\begin{theorem}
\label{thm:tk1}
\TKC\ is fixed-parameter tractable.
\end{theorem}

==> figs/2k2.tex <==
\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
    \node (o) at (0,0) {};
    \node[myv] (v1) at (-0.15,0.15) {};
    \node[myv] (v2) at (-0.15,-0.15) {};
    \node[myv] (v3) at (0.15,0.15) {};
    \node[myv] (v4) at (0.15,-0.15) {};

    \draw (v1) -- (v2);
    \draw (v3) -- (v4);
\end{tikzpicture}


==> figs/diamond.tex <==
\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
    \node (o) at (0,0) {};
    \node[myv] (v1) at (0,0.15) {};
    \node[myv] (v2) at (0,-0.15) {};
    \node[myv] (v3) at (-0.3,0) {};
    \node[myv] (v4) at (0.3,0) {};

    \draw (v1) -- (v2);
    \draw (v1) -- (v3);
    \draw (v1) -- (v4);
    \draw (v2) -- (v3);
    \draw (v2) -- (v4);

\end{tikzpicture}


==> figs/k2k1.tex <==
\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
    \node (o) at (0,0) {};
    \node[myv] (v1) at (-0.15,0.15) {};
    \node[myv] (v2) at (-0.15,-0.15) {};
    \node[myv] (v3) at (0.15,0) {};

    \draw (v1) -- (v2);
\end{tikzpicture}


==> whardness/disconnected.tex <==
\subsection{Disconnected graphs}

==> whardness/general-1.tex <==
\subsubsection{Graphs containing $K_2+K_1$ but no false twins}
Let $H$ be a graph having an induced $K_2+K_1$ but no false twins. We prove that \HFC\ is W[2]-hard by a parameterized reduction from \DS.
Let  $V(H) = \{u_1, u_2, \ldots, u_t\}$. Without loss of generality, assume that $\{u_1,u_2,u_3\}$ induces a $K_2+K_1$ and $u_1u_2$ is an edge in the $K_2+K_1$.

Let $(G',k)$ be an instance of \DS.
Let $V(G')=\{ v_1, v_2, \ldots , v_n \}$. Then, $G$ is constructed as per the following steps (see Figure \ref{fig:2K2}):
%\input{hardness/small/2K2-figure}

\begin{enumerate}[(i)]
    \item The vertices of $G$ consists of $t$ independent sets $I_1, I_2,\ldots, I_t$. The set $I_1$ has a single vertex $w$,
    $I_2$ and $I_3$ has $n$ vertices each and the rest of the sets have $k+1$ vertices each.
    
    \item Let $X=I_2=\{ x_1, x_2, \ldots , x_n \}$ and $Y=I_3=\{ y_1, y_2, \ldots , y_n \}$.  
    For $1\leq i,j\leq n$, there exists an edge $x_iy_j$ if and only if $i=j$ or $v_iv_j \in E(G')$.
    
    \item For every pair of sets $I_i, I_j$, except for the pair $I_2,I_3$, the adjacency is as follows: every vertex in $I_i$
    is adjacent to every vertex in $I_j$ if $u_i$ and $u_j$ are adjacent in $H$, and $I_i$ and $I_j$ together form an independent set otherwise.
\end{enumerate}

\begin{lemma}
\label{lem:k3uk1-if}
Let $(G',k)$ be a yes-instance of \DS. Then $(G,k)$ is a yes-instance of \HFC.
\end{lemma}
\begin{proof}
Let $D$, of size at most $k$, be a dominating set of $G'$. Let $\mathcal{P}$ be a partition of the vertices of $G$ such that it 
consists of a set $P$ containing $w$ and $x_i$ for every $v_i$ in $D$.
Every other set in $\mathcal{P}$ is a singleton set. We claim that $G'' = G/\mathcal{P}$ is $H$-free.
We note that the vertices in $G''$ can be partitioned into $t$ independent sets $I_1', I_2',\ldots, I_t'$, where $I_1'=\{w\}$, 
$I_2'$ is obtained from removing vertices in $P$ from $I_2$, and for the rest of the sets, $I_i' = I_i$. We also note that
$I_i'$ is a module. To prove that $G''$ is $H$-free, for a contradiction, assume that there is an $H$ induced by a set $V'$ in $G''$. 
Since $H$ does not have any false twins, $V$ contains only at most one vertex from each set $I_i'$. 
Then $V'$ contains exactly one vertex from each set $I_i'$ and hence $V'$ induces a graph having at least one more edge than that in $H$ - 
note that $w$ is adjacent to $I_2'$ in $G''$ and not adjacent to $I_2$ in $G$. 
Thus we get a contradiction.
\end{proof}

\begin{lemma}
\label{lem:k3uk1-onlyif}
Let $(G,k)$ be a yes-instance of \HFC. Then $(G',k)$ is a yes-instance of \DS.
\end{lemma}
\begin{proof}
Let $\mathcal{P}$ be a solution of $(G,k)$. Let $X'$ be the set of all vertices in $X$ part of some non-singleton set in $\mathcal{P}$.
We can safely assume that $G'$ is connected and is not a complete graph. Then we claim that $X'$ is nonempty. For a contradiction, assume that $X'$
is empty. Let $v_iv_j$ be any nonedge in $G'$.
Form a set $Z$ by taking exactly one arbitrary vertex $z_q$ from $I_q$, for $4\leq q\leq t$, 
such that $z_q$ is not part of any non-singleton set in $\mathcal{P}$ - 
there exists such a vertex as $I_q$ (for $4\leq q\leq t$) 
is an independent set of size $k+1$ and \cost{\mathcal{P}} is at most $k$. Then $Z\cup \{w, x_i, y_j\}$ induces an $H$,
which is a contradiction. Therefore, $X'$ is nonempty. We are going to construct a dominating set $D$ for $G'$ from $X'$. If every vertex in $Y$
is adjacent to at least one vertex in $X'$, then we set $D$ as the set of vertices in $G'$ corresponding to the vertices in $X'$, i.e., 
$D = \{v_i \mid x_i \in X'\}$. If there exists a vertex in $Y$ not adjacent to any vertex in $X'$, then we set $D$ as follows. Let $x_j$ be any 
vertex in $X'$ such that $v_j$ has a neighbor $v_\ell$ and $x_\ell$ not in $X'$. 
There exists such a vertex as $G'$ is connected. Now, let $X''$ be $(X'\setminus \{x_j\})\cup \{x_\ell\}$.
Then we set $D$ to be the vertices in $G'$ corresponding to the vertices in $X''$, i.e., $D = \{v_i\mid x_i\in X''\}$.
Now we claim that, in both the cases, $D$ is a dominating set of size at most $k$. 
First we claim that $D$ has at most $k$ vertices. Let $P$ be any non-singleton set in $\mathcal{P}$
containing at least one vertex in $X$. Since $X$ is an independent set and $P$ induces a connected graph in $G$, we obtain that \cost{P} is at least
the number of vertices in $X\cap P$. Therefore, $|D|\leq k$. It remains to show that $D$ is a dominating set of $G'$. For a contradiction, 
assume that there is a vertex $v_i\in V(G')\setminus N[D]$. Then, clearly, $D$ is obtained from $X''$.
Assume that $D$ is not a dominating set. Then there is a vertex $v_q$ not in $D$ and not adjacent to any vertex in $D$. 
This implies that $v_q$ is not in $D$ and none of the vertices in $D$, in particular $v_\ell$, is not adjacent to $v_q$. 
Then $\{u,x_\ell,x_q,z\}$ induces an $H$ in $G/\mathcal{P}$, where $z$ is any vertex in $Z$ such that $z$ is not part of any non-singleton set in $\mathcal{P}$ - 
such a vertex exists as $Z$ is an independent set of size $k+1$ and \cost{\mathcal{P}} is at most $k$.
\end{proof}

==> whardness/hardness-small.tex <==
\subsection{Small graphs}
\input{hardness/small/k2uk1.tex}
%\input{hardness/small/2K2}
%\input{hardness/small/claw}
%\input{hardness/small/T12}
%\input{hardness/small/K3UK1}

==> whardness/small/2K2-figure.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
  \node (c) at (0,0) {};

  \node[myv,label=above:$u$] (u) at (-2,0) {};
  \node[myv,label=above:$x_i$] (x1) at (-1,0.5) {};
  \node[myv,label=below:$x_j$] (x2) at (-1,-0.5) {};
  \node[myv,label=above:$y_i$] (y1) at (1,0.5) {};
  \node[myv,label=below:$y_j$] (y2) at (1,-0.5) {};
  \node[myv] (z11) at (2.5,1) {};
  \node[myv] (z12) at (2.5,0.5) {};
  \node[myv] (z21) at (2.5,-0.5) {};
  \node[myv] (z22) at (2.5,-1) {};

%  \draw (u) --node[below] {e} ++(v);

  \draw (u) -- (x1);
  \draw (u) -- (x2);
  %\draw (y1) -- (x1);
  %\draw (y1) -- (x2);
  %\draw (y2) -- (x1);
  %\draw (y2) -- (x2);
  \draw (y1) -- (y2);
  \draw (y1) -- (z11);
  \draw (y1) -- (z12);
  \draw (y2) -- (z21);
  \draw (y2) -- (z22);
  \draw[dashed, red] (0.5, 1.25) rectangle (1.5, -1.25);
  \node (x) at (-1,-1.5) {$X$};
  \draw [dashed, red] (-1, 0) ellipse (0.5 and 1.25);
  \node (y) at (1,-1.5) {$Y$};
  \draw[dashed, red] (2.5, 0.75) ellipse (0.25 and 0.6);
  \node (z1) at (3.0,0.75) {$Z_i$};
  \draw[dashed, red] (2.5, -0.75) ellipse (0.25 and 0.6);
  \node (z1) at (3.0,-0.75) {$Z_j$};
  \draw[decorate,decoration=snake] (-0.5,0) -- (0.5,0);


%  \draw[dashed, red, fill=red!15, opacity=0.45] (0, -1.5) ellipse (0.6 and 0.6);
%  \node[blue] (w) at (0,-1.9) {$W$};  
%  \draw[dashed, red, fill=red!15, opacity=0.45] (-1.25, 0.875) ellipse (0.6 and 0.6);
%  \node[blue] (x) at (-1.5,1.15) {$X_e$};
%  \draw[dashed, red, fill=red!15, opacity=0.45] (1.25, 0.875) ellipse (0.6 and 0.6);
%  \node[blue] (y) at (1.5,1.15) {$Y_e$};
%  \draw[dashed, red, fill=red!15, opacity=0.45] (0, 1.75) ellipse (0.6 and 0.6);
%  \node[blue] (z) at (-0.3,1.9) {$Z_e$};
\end{tikzpicture}
    \caption{Construction of instance $(G,k)$ of {\sc $2K_2$-Free Contraction} from the instance $(G',k)$ of {\sc Dominating Set}. Rectangle represents a clique and ellipse represents an independent set. Adjacency between $X$ and $Y$ depends on the edges of $G'$.}
    \label{fig:2K2}
\end{figure}

==> whardness/small/2K2-old.tex <==
\subsubsection{$2K_2$}

For the rest of this subsection, we assume that $H \cong 2K_2$. With that assumption, we prove that the problem of {\sc $H$-Free Contraction} is $W[2]$-hard. To prove so, we give a parameterized reduction from \DS.

\medskip

Let $(G',k)$ be an instance of \DS.
Let $V(G')=\{ v_1, v_2, \ldots , v_n \}$. Then, $G$ is constructed in the following steps (refer to Figure \ref{fig: 2K2}):
\input{hardness/small/2K2 figure}

\begin{enumerate}
    \item Let $X=\{ x_1, x_2, \ldots , x_n \}$, $Y=\{ y_1, y_2, \ldots , y_n \}$ and that $x_ix_j$ and $x_iy_i$ be edges for all $1 \leq i,j \leq n$. Moreover, let $x_iy_j$ be an edge if and only if $v_iv_j \in E(G')$.
    
    \item For each $x_i \in X$, let $Z_i$ be a set of $k+1$ vertices and that $x_iz$ be edges for all $i$ and all $z \in Z_i$. 
    
    \item Let $A=\{ a_1, a_2, \ldots , a_{k+1} \}$ and $u$ be a vertex and that $ua_i$ and $uy_i$ be edges for all $i$.
\end{enumerate}

\begin{lemma} \label{lem_2K2_Dom Set -> H-Free}
Let $(G',k)$ be a yes-instance of {\sc Dominating Set}. Then, $(G,k)$ is a yes-instance of {\sc $H$-Free Contraction}.
\end{lemma}

\begin{proof}
Since $(G',k)$ is a yes-instance of {\sc Dominating Set}, let $T' \subset V(G')$ such that $|T'| \leq k$ and that $T'$ is a dominating set of $G'$. Let $T=\{ y_j \in Y: v_j \in T' \}$ and $S=\{ uy: y \in T \} \subset V(G)$. We claim that $S$ is a solution of $(G,k)$.

\medskip

Since $x_iu$ are edges in $G/S$ for all $i$, and the subgraph of $G$ induced by $X$ is a clique, $G/S$ is clearly $H$-free. Moreover, $|S|=|T|=|T'| \leq k$ and hence, $S$ is a solution of $(G,k)$.
\end{proof}

\begin{lemma} \label{lem_2K2_H-Free -> Dom Set}
Let $(G,k)$ be a yes-instance of {\sc $H$-Free Contraction}. Then, $(G',k)$ is a yes-instance of {\sc Dominating Set}.
\end{lemma}

\begin{proof}
To prove that $(G',k)$ is a yes-instance of {\sc Dominating Set}, it is enough to show that for any solution $S$ of $(G,k)$ and for all $x_i \in X$, there exists a $y_j \in T_u=\{ y \in Y: uy \in S \} \cup \{ u \}$ such that $x_iy_j \in E(G)$. In this case, $T'= \{ v_j \in V(G'): y_j \in T_u \}$ is a dominating set of $G'$. Moreover, since $|T'|=|T_u|-1 \leq |S| \leq k$, $T'$ is a solution of $(G',k)$. 

\medskip

So, let $S$ be a minimal solution of $(G,k)$ such that $S \cap E[Y, \{ u \}]$ is maximal. We claim that $S \cap E[X, X \cup Y] = \emptyset$. If not, let $x_iw \in S \cap E[X, X \cup Y]$ for some $w \in X \cup Y$. We then construct a new subset $S_1$ of $E(G)$ by $S_1= (S \setminus \{ x_iw \}) \cup \{ uy_i \}$ and claim that $S_1$ is also a a solution of $(G,k)$. Firstly, $|S_1|=|S| \leq k$. So, toward a contradiction, if there exist $p, q, r, s \in V(G)$ such that $\{ p, q, r, s \}$ induces a $2K_2$ in $G/S_1$ with $pq$ and $rs$ being edges in the $2K_2$, then, without loss of generality, it can happen with $p=x_j \in X$, $q \in Z_j$, $r \in A$ and $s=u$. Let $T_p$ be the set of vertices in $V(G)$ which contract to $p$ in $G/S$. Then, $x_i \in T_p $. Now, since $x_iy_i \in E(G)$, $ps \in E(G/S_1)$. This is a contradiction. Hence, $(G/S_1)$-free and thus, $S_1$ is a solution of $(G,k)$. However, this is again a contradiction, as $S_1$ is minimal and $|S_1 \cap E[Y, \{ u \}]| = |S \cap E[Y, \{ u \}]|+1$. This establishes our claim that $S \cap E[X, X \cup Y] = \emptyset$.

\medskip

Now, given that such an $S$ is minimal, we must have $S \cap E[\{ x_i \}, Z_i] = \emptyset$ for all $i$ and $S \cap E[\{ u \}, A] = \emptyset$ as well. This implies that $S \subset E[Y, \{ u \}]$, which further implies that for all $x_i \in X$, there exists a $y_j \in T_u$ such that $x_iy_j \in E(G)$. Hence, we are done.
\end{proof}

Thus, putting together Lemmas \ref{lem_2K2_Dom Set -> H-Free} and \ref{lem_2K2_H-Free -> Dom Set}, we have:

\begin{theorem}
For $H \cong 2K_2$, {\sc $H$-Free Contraction} is $W[2]$-hard.
\end{theorem}

==> whardness/small/2K2.tex <==
\subsubsection{$2K_2$}

\begin{observation}
    \label{obs:2k2}
    Let $S$ be a subset of edges of a graph $G$. Let $S'$ be a subset of $S$.
    If $G/S$ has an induced $2K_2$, then there is an induced $2K_2$ in $G/S'$.
\end{observation}
\begin{proof}
Let $\mathcal{P}$ and $\mathcal{P'}$ be the partitions induced by $S$ and $S'$ respectively. Assume that $\{P_a, P_b, P_c, P_d\}\subseteq \mathcal{P}$
induces a $2K_2$ in $G/S$, where $P_aP_b$ and $P_cP_d$ are the edges of 
the $2K_2$. If $\mathcal{P} = \mathcal{P'}$, then we are done. Otherwise,
$\mathcal{P'}$ is a refinement of $\mathcal{P}$. Therefore, there exists $P'_{a'}\subseteq P_a$ and $P'_{b'}\subseteq P'_b$ such that $P'_{a'}$ and $P'_{b'}$ are adjacent in $G/S'$, and there exist $P'_{c'}\subseteq P_c$ and 
$P_{d'}\subseteq P_d$ such that $P'_{c'}$ and $P'_{d'}$ are adjacent in $G/S'$. Since neither $P_a$ nor $P_b$ is adjacent to neither $P_c$ nor $P_d$ in $G/S$, we obtain that neither $P'_{a'}$ nor $P'_{b'}$ is adjacent to 
neither $P'_{c'}$ nor $P'_{d'}$ in $G/S'$. Therefore, $\{P'_{a'}, P'_{b'}, P'_{c'}, P'_{d'}\}$ induces a $2K_2$ in $G/S'$.
\end{proof}

Let $(G',k)$ be an instance of \DS.
Let $V(G')=\{ v_1, v_2, \ldots , v_n \}$. Then, a graph $G$ is constructed as follows:
\input{hardness/small/2K2-figure}

\begin{enumerate}[(i)]
    \item Introduce two sets $X=\{ x_1, x_2, \ldots , x_n \}$, $Y=\{ y_1, y_2, \ldots , y_n \}$ of vertices, where $X$ forms an independent set and $Y$ forms a clique.
    Introduce an edge $x_iy_j$ if and only if $i=j$ or $v_iv_j$ is an edge in $G'$.
    \item For each $y_i \in Y$, introduce an independent set $Z_i$ of $k+1$ vertices and make $y_i$ adjacent to all vertices in $Z_i$.
    
    \item Introduce a vertex $u$ and make it adjacent to all vertices in $X$.
\end{enumerate}

Let $Z$ be the union of all $Z_i$s. This completes the construction (see Figure \ref{fig:2K2}). 

\begin{observation}
    \label{obs:2k2-type}
    Every induced $2K_2$ in $G$ is either formed by two edges $ux$ and $yz$
    (for some $x\in X, y\in Y, z\in Z$) or formed by two edges $ux$ and $yy'$
    (for some $x\in X, y,y'\in Y$).
\end{observation}

\begin{lemma} \label{lem_2K2_Dom Set -> H-Free}
Let $(G',k)$ be a yes-instance of \DS. Then, $(G,k)$ is a yes-instance of \XFC{2K_2}.
\end{lemma}

\begin{proof}
Let $T' \subseteq V(G')$ be such that $|T'| \leq k$ and that $T'$ is a dominating set of $G'$. 
Let $S=\{ux_j: v_j \in T'\}$. We claim that $S$ is a solution of $(G,k)$.

Clearly $|S|=|T'|\leq k$. It remains to prove that $G/S$ is $2K_2$-free. Let $\mathcal{P}$ be the partition induced by $S$. We observe 
that the only non-singleton set $P_u$ in $\mathcal{P}$ is formed by the end vertices, which include $u$, 
of edges in $S$. Since $T'$ is a dominating set of $G'$, $P_u$ is adjacent to every set $P_y$, corresponding to the vertices in $Y$, in $G/S$. Now, it is straight-forward to verify that $G/S$ is a split graph, where a clique is formed by $P_u$ and the sets corresponding to vertices in $Y$, and the remaining vertices form an independent set. 
Therefore, $G/S$ is $2K_2$-free.
%By construction, the vertex $u$ is adjacent to every vertex in $X$.
%Since $T'$ is a dominating set of $G'$, the vertex $u$ is adjacent to every vertex in $Y$ in $G/S$. Therefore, $u$ cannot be part of an induced $2K_2$. Now, every edge not incident to $u$ has at least one end point in $Y$, which forms a clique. Moreover, $G/S$ is a split graph. Therefore, we obtain that $G/S$ is $2K_2$-free.
\end{proof}

\begin{lemma} \label{lem_2K2_H-Free -> Dom Set}
Let $(G,k)$ be a yes-instance of \XFC{2K_2}. Then, $(G',k)$ is a yes-instance of \DS.
\end{lemma}

\begin{proof}
Let $S$ be a minimum solution of $(G,k)$ having minimum number of $x_iy_j$ type edges among all minimum solutions. Due to minimality of $S$ and abundance of edges of type $y_iz$ (for $z\in Z_i$), $S$ does not contain any edge of type $y_iz$. 

Claim 1: $S$ does not contain any edge of type $x_iy_j$. 

For a contradiction, assume that $S$ has an edge $x_py_q$. 
Create a new set $S'$ from $S$ by: 
\[\text{replacing } x_py_p\ \text{with} 
\begin{cases}
ux_p, & \text{if } ux_p\notin S\\
ux_q, & \text{otherwise}
\end{cases}
\]
%replacing $x_py_q$ with $ux_p$, if . 
Clearly, $|S'|\leq |S|$. We claim that $G/S'$ is $2K_2$-free, contradicting the minimality 
(with respect to the number of edges of type $x_iy_j$) of $S$. 
Let $\mathcal{P}$ and $\mathcal{P'}$ be the partitions induced by $S$ and $S'$ respectively.
Let $S'' = S\setminus \{x_py_q\}$. Since $S$ is a minimal solution, $S$ forms a forest in $G$, by Observation~\ref{obs:solution-forest}.
Therefore, the partition $\mathcal{P''}$ induced by $S''$ is same as the 
partition $P$, except that for two sets $P''_{x_p}$ and $P''_{y_q}$ in $\mathcal{P''}$, there is a single set $P_{x_p} = P_{y_q} = P''_{x_p}\cup P''_{y_q}$ in $\mathcal{P}$.
%If $G/S''$ does not have any induced $2K_2$, then by Observation~\ref{obs:2k2}, $G/S'$ does not have any induced $2K_2$. 
Clearly, $G/S''$ has an induced $2K_2$ (if not, then $S$ is not a minimum solution).
%Therefore, assume that $G/S''$ has an induced $2K_2$. 
By Observation~\ref{obs:2k2-type}, the edges of an induced $2K_2$ in $G$ are of the form $ux$, $yz$ or of the form $ux$, $yy'$ (for some $x\in X, y,y'\in Y, z\in Z$). 
Therefore, the edges of induced $2K_2$s in $G/S''$ are of the form $P''_uP''_x$, $P''_yP''_z$ or of the form $P''_uP''_x$, $P''_yP''_{y'}$ (for some $x\in X, y,y'\in Y, z\in Z$).
Since $S''$ does not contain any edges of type $yz$, if there is a $2K_2$ of later type in $G/S''$, then there is a $2K_2$ of the former type in $G/S''$. Therefore, we can safely assume that this $2K_2$ is formed by two edges 
$P''_uP''_x$ and $P''_yP''_z$, for some vertices $x\in X, y\in Y$, and $z\in Z$. 
We observe the following:
\begin{itemize}
    \item $P''_u$ may contain vertices from $X$ but not from $Y\cup Z$: If it contains vertices from $Y$ then $P''_u$ and $P''_y$ are adjacent. Since it does not contain vertices from $Y$, it cannot contain vertices from $Z$.
    \item $P''_x = \{x\}$: Clearly, $P''_x$ does not contain $u$. If it contains a vertex from $Y$, then it is adjacent to $P''_y$. Since it does not contain vertices from $Y\cup \{u\}$, it cannot 
    contain vertices from $X\cup Z$.
    \item $P''_y\subseteq Y$: Since $S''$ does not contain any edge of type $y_iz$, $P''_y$ cannot contain any vertex from $Z$. Further, if $P''_y$ contains a vertex from $X$, it becomes adjacent to $P''_u$.
    \item $P''_z=\{z\}$: Since $S''$ does not contain any edge of type $y_iz$, $P''_z$ cannot contain vertices from $Y$.
    Therefore, it cannot contain any other vertex.
\end{itemize}
Since there is no edge between $P''_x$ and $P''_y$, it is not true that both $x_p\in P''_x\cup P''_y$ and $y_q\in P''_x\cup P''_y$ are true. But, since $G/S$ is $2K_2$-free, either $x_p\in P''_x\cup P''_y$ or $y_q\in P''_x\cup P''_y$. 
If $P''_x$ contains any vertex from $Y$, then $P''_x$ becomes 
adjacent to $P''_y$, as $Y$ is a clique. Therefore, $P''_x$ does not contain any vertex from $Y$. 
Therefore, $x_p\in P''_x\cup P''_y$ or $y_p\in P''_y$.
Assume that $x_p\in P''_x\cup P''_y$. Since $S'$ contains $ux_p$, 
we obtain that either $P'_u = P'_x$ or $P'_u= P'_y$. Therefore, the $2K_2$ does not exists in $G/S'$. Assume that $y_q\in P''_y$. Then $P'_u$ is adjacent to $P'_y$ in $G/S'$. Therefore, the $2K_2$ does not exist in $G/S'$.

Thus we obtain that $S$ can contains only edges of types $ux_i$ and $y_jy_\ell$. This implies that $P_u, P_{x_i}\subseteq X\cup \{u\}$, and $P_{y_j}\subseteq Y$. 

Claim 2: For every $P\in \mathcal{P}$ such that $P\subseteq Y$, there is an edge $ux_i$ in $S$
such that $x_i$ is adjacent to at least one vertex in $P$ in $G$.

For a contradiction, assume that there is a set $P\in \mathcal{P}$ such that there are no edges of type $ux_i$ in $S$ such that $x_i$ is adjacent to at least one vertex in $P$. Then $\{u,x_i,y_j, z\}$ induces a $2K_2$ in $G/S$, where $x_i$ is any vertex in $X$ such that $ux_i\notin S$ (there exists such a vertex, as we can safely assume that $k < n$), $y_j\in P$, and $z\in Z_j$.

With Claim 1 and 2, we are ready to prove the statement of the lemma. 
From $S$, we create a dominating set $T'$ of size at most $k$ of $G'$.
For every $ux_j$ type edge in $S$, include $v_j$ in $T'$. For every $P_i\in \mathcal{P}$ such that $P\subseteq Y$,
let $x_i$ (without loss of generality) be the vertex in $X$, as per Claim 2, such that $ux_i\in S$ and $x_i$ is adjacent to at least one vertex, say $y_j$, in $P_i$. Include in $T'$ the edges $ux_\ell$ for every vertex $y_\ell$ in $P\setminus \{y_j\}$.  
We note that there are exactly $|P_i|-1$ edges of $G$ in $S$. For each 
vertex $y_\ell$ in $P_i$, there is a vertex adjacent ($x_\ell$ if $\ell\neq j$ and $x_i$ if $\ell = j$) to it in $X$ such that the corresponding vertex in $G'$ is added to $T'$. Therefore, $|T'|\leq |S|\leq k$ and $T$ is a dominating set of $G$.
\end{proof}

Thus, putting together Lemmas \ref{lem_2K2_Dom Set -> H-Free} and \ref{lem_2K2_H-Free -> Dom Set}, we have:

\begin{theorem}
\XFC{2K_2} is $W[2]$-hard.
\end{theorem}

==> whardness/small/2K2_figure-old.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[scale=1.5]
    
    \node at (-0.5,-0.5) {$X$};
    \fill (0.5,-0.5) circle (2pt) node[left] {$x_i$};
    \fill (1.5,-0.5) circle (2pt) node[right] {$x_j$};
    
    \node at (-0.5,-3.5) {$Y$};
    \fill (0.5,-3.5) circle (2pt) node[below] {$y_i$};
    \fill (1.5,-3.5) circle (2pt) node[below] {$y_j$};
    
    \fill (5.5,-0.5) circle (2pt) node[above] {$a_i$};
    \fill (6.5,-0.5) circle (2pt) node[above] {$a_j$};
    
    \draw (0.5,-0.5) -- (1.5,-0.5);
    \draw (0.5,-0.5) -- (1.5,-3.5);
    \draw (0.5,-3.5) -- (1.5,-0.5);
    \draw (0.5,-0.5) -- (0.5,-3.5);
    \draw (1.5,-0.5) -- (1.5,-3.5);
    
    \node at (7.5,-0.5) {$A$};
    \node at (7.5,-3.5) {$B$};
    \fill (3.5,-2) circle (2pt) node[above left] {$u$};
    
    \draw[very thick] (3.5,-2) -- (5.5,-0.5);
    \draw[very thick] (3.5,-2) -- (6.5,-0.5);
    
    \draw[very thick] (3.5,-2) -- (0.5,-3.5);
	\draw[very thick] (3.5,-2) -- (1.5,-3.5);    
    
    \draw (0,0) -- (2,0);
    \draw (0,0) -- (0,-1);
    \draw (2,0) -- (2,-1);
    \draw (0,-1) -- (2,-1);
    
    \draw (0,-3) -- (2,-3);
    \draw (0,-3) -- (0,-4);
    \draw (2,-3) -- (2,-4);
    \draw (0,-4) -- (2,-4);
    
    \draw (5,0) -- (7,0);
    \draw (5,0) -- (5,-1);
    \draw (7,0) -- (7,-1);
    \draw (5,-1) -- (7,-1);
    
    \draw (0.25,1) -- (0.75,1);
    \draw (0.25,1.5) -- (0.75,1.5);
    \draw (0.25,1) -- (0.25,1.5);
    \draw (0.75,1) -- (0.75,1.5);
    
    \draw (1.25,1) -- (1.75,1);
    \draw (1.25,1.5) -- (1.75,1.5);
    \draw (1.25,1) -- (1.25,1.5);
    \draw (1.75,1) -- (1.75,1.5);
    
    \node at (0,1.25) {$Z_i$};
    \node at (2,1.25) {$Z_j$};
    
    \fill (0.5,1.25) circle (2pt) node {};
    \fill (1.5,1.25) circle (2pt) node {};
    
    \draw[very thick] (0.5,-0.5) -- (0.5,1.25);
    \draw[very thick] (1.5,-0.5) -- (1.5,1.25);

    \end{tikzpicture}
    \caption{Construction of instance $(G,k)$ of {\sc $2K_2$-Free Contraction} from the instance $(G',k)$ of {\sc Dominating Set}. The thick edges represent ``all edges".}
    \label{fig: 2K2}
\end{figure}

==> whardness/small/K3UK1.tex <==
\subsubsection{$K_3\cup K_1$}
Let $H$ be $K_3\cup K_1$. We prove that \HFC\ is W[2]-hard by a parameterized reduction from \DS.

Let $(G',k)$ be an instance of \DS.
Let $V(G')=\{ v_1, v_2, \ldots , v_n \}$. Then, $G$ is constructed as per the following steps (see Figure \ref{fig:2K2}):
%\input{hardness/small/2K2-figure}

\begin{enumerate}[(i)]
    \item The vertices of $G$ consists of three independent sets $X, Y, Z$, and a vertex $u$. The sets
    $X$ and $Y$ have $n$ vertices each and $Z$ has $k+1$ vertices.
    \item Let $X=\{ x_1, x_2, \ldots , x_n \}$ and $Y=\{ y_1, y_2, \ldots , y_n \}$.  
    For $1\leq i,j\leq n$, there exists an edge $x_iy_j$ if and only if $i=j$ or $v_iv_j \in E(G')$.
    
    \item Every vertex in $X$ is adjacent to every vertex in $Z$.
    
    \item The vertex $u$ is adjacent to every vertex in $X\cup Z$.
\end{enumerate}

\begin{lemma}
\label{lem:k3uk1-if}
Let $(G',k)$ be a yes-instance of \DS. Then $(G,k)$ is a yes-instance of \HFC.
\end{lemma}
\begin{proof}
Let $D$, of size at most $k$, be a dominating set of $G'$. Let $\mathcal{P}$ be a partition of the vertices of $G$ such that it 
consists of a set $P$ containing $u$ and $x_i$ for every $v_i$ in $D$.
Every other set in $\mathcal{P}$ is a singleton set. We claim that $G'' = G/\mathcal{P}$ is $H$-free. 
Clearly, $v$ is adjacent to every other vertex in $G''$. Therefore, $v$ cannot be a part of any induced $H$ in $G''$. Further, 
$G''-v$ is a bipartite graph having the bipartition $X$ and $Y\cup Z$. Therefore, there exists no induced $H$ in $G''$.
\end{proof}

\begin{lemma}
\label{lem:k3uk1-onlyif}
Let $(G,k)$ be a yes-instance of \HFC. Then $(G',k)$ is a yes-instance of \DS.
\end{lemma}
\begin{proof}
Let $\mathcal{P}$ be a solution of $(G,k)$. Let $X'$ be the set of all vertices in $X$ part of some non-singleton set in $\mathcal{P}$.
We can safely assume that $G'$ is connected and is not a complete graph. Then we claim that $X'$ is nonempty. For a contradiction, assume that $X'$
is empty. Let $v_iv_j$ be any nonedge in $G'$. Let $z$ be any vertex in $Z$ such that $z$ is not part of any non-singleton set in $\mathcal{P}$ - 
there exists such a vertex as $Z$ is an independent set of size $k+1$ and \cost{\mathcal{P}} is at most $k$. Then $\{u,z,x_i,y_j\}$ induces an $H$,
which is a contradiction. Therefore, $X'$ is nonempty. We are going to construct a dominating set $D$ for $G'$ from $X'$. If every vertex in $Y$
is adjacent to at least one vertex in $X'$, then we set $D$ as the set of vertices in $G'$ corresponding to the vertices in $X'$, i.e., 
$D = \{v_i \mid x_i \in X'\}$. If there exists a vertex in $Y$ not adjacent to any vertex in $X'$, then we set $D$ as follows. Let $x_j$ be any 
vertex in $X'$ such that $v_j$ has a neighbor $v_\ell$ and $x_\ell$ not in $X'$. 
There exists such a vertex as $G'$ is connected. Now, let $X''$ be $(X'\setminus \{x_j\})\cup \{x_\ell\}$.
Then we set $D$ to be the vertices in $G'$ corresponding to the vertices in $X''$, i.e., $D = \{v_i\mid x_i\in X''\}$.
Now we claim that, in both the cases, $D$ is a dominating set of size at most $k$. 
First we claim that $D$ has at most $k$ vertices. Let $P$ be any non-singleton set in $\mathcal{P}$
containing at least one vertex in $X$. Since $X$ is an independent set and $P$ induces a connected graph in $G$, we obtain that \cost{P} is at least
the number of vertices in $X\cap P$. Therefore, $|D|\leq k$. It remains to show that $D$ is a dominating set of $G'$. For a contradiction, 
assume that there is a vertex $v_i\in V(G')\setminus N[D]$. Then, clearly, $D$ is obtained from $X''$.
Assume that $D$ is not a dominating set. Then there is a vertex $v_q$ not in $D$ and not adjacent to any vertex in $D$. 
This implies that $v_q$ is not in $D$ and none of the vertices in $D$, in particular $v_\ell$, is not adjacent to $v_q$. 
Then $\{u,x_\ell,x_q,z\}$ induces an $H$ in $G/\mathcal{P}$, where $z$ is any vertex in $Z$ such that $z$ is not part of any non-singleton set in $\mathcal{P}$ - 
such a vertex exists as $Z$ is an independent set of size $k+1$ and \cost{\mathcal{P}} is at most $k$.
\end{proof}

==> whardness/small/T12.tex <==
\subsubsection{$T_{1,2}$}

In this section we prove that, when $H$ is the bistar graph $T_{1,2}$, \HFC\ is $W[2]$-hard by a reduction from \DS.
Given an instance $(G',k)$ of \DS, we construct a graph $G$ such that $(G',k)$ is a yes-instance of \DS\ if and only if
$(G,k)$ is a yes-instance of \HFC. Let $V(G') = \{v_1,v_2,\ldots, v_n\}$. The construction is described below. 

\begin{itemize}
    \item Introduce five sets $X,Y,A,B,C$ of vertices such that each set forms a clique. Further, $X$ and $Y$ have $n$ vertices each
    and $A,B,$ and $C$ have $k+1$ vertices each. Additionally, introduce a vertex $u$.
    \item Let $X = \{x_1, x_2, \ldots, x_n\}$ and $Y=\{y_1, y_2,\ldots, y_n\}$. Add an edge $x_iy_j$ if and only if $i=j$ or $v_iv_j\in E(G')$.
    Every vertex in $A$ is adjacent to every vertex in $B\cup Y$ and every vertex in $B$ is adjacent to every vertex in $C$.
    The vertex $u$ is adjacent to every vertex in $X\cup A$.
\end{itemize}

\begin{lemma}
\label{lem:t12-forward}
If $(G',k)$ is a yes-instance of \DS, then $(G,k)$ is a yes-instance of \HFC.
\end{lemma}
\begin{proof}
Let $T'$ be a dominating set of $G'$ such that $|T'|\leq k$. 
Let $T$ be the vertices in $X$ corresponding to the vertices in $T'$, i.e., $T=\{x_i\mid v_i\in T'\}$.
Let $\mathcal{P}$ be a partition where the only non-singleton set be $P=T\cup \{u\}$. It can be easily verified that
there is no vertex in $G/\mathcal{P}$ having an independent set of size 3 in its neighborhood. Therefore, $G/\mathcal{P}$
is $H$-free.
\end{proof}

\begin{observation}
\label{obs:t12-backward}
Let $J$ be the graph induced by $X\cup Y$ in $G$.
Let $\mathcal{P}$ be a partition of the vertices of $J$ such that every set in $\mathcal{P}$
is either a subset of $X$ or a subset of $Y$ and that $J/\mathcal{P}$ is a complete graph.
Then $|\mathcal{P}|\geq k+1$.
\end{observation}
\begin{proof}
For a contradiction, assume that $|\mathcal{P}|\leq k$. 

\end{proof}

\begin{lemma}
\label{lem:t12-backward}
If $(G,k)$ is a yes-instance of \HFC, then $(G',k)$ is a yes-instance of \DS.
\end{lemma}
\begin{proof}
Let $\mathcal{P}$ be a partition of vertices of $G$ such that $G/\mathcal{P}$ is $H$-free and \cost{\mathcal{P}} is at most $k$.
It is straight-forward to verify that there exists sets $P_A\subseteq A, P_B\subseteq B$, and $P_C\subseteq C$ in $\mathcal{P}$
such that $P_AP_BP_C$ induces a $P_3$ in $G/\mathcal{P}$.
Let $P_u$ be the set containing $u$.
We split the proof into two cases.

Case 1: $P_u$ does not contain any vertex from $A$.

If $P_u$ is not equal to and not adjacent to a set $P_Y$ containing at least one vertex from $Y$,
then $\{P_u, P_Y, P_A, P_B, P_C\}$ induces a $T_{1,2}$, which is a contradiction. 
Therefore, $P_u$ is equal to or adjacent to every set containing 
vertices from $Y$. We construct a set $T\subseteq X$ as follows. 
\begin{enumerate}[(i)]
\item For every set $P$ in $\mathcal{P}$ containing at least one vertex from $X$ and 
at least one vertex from $Y\cup \{u\}$, do the following: 
Let $x_\ell$ be a vertex in $P\cap X$ such that $x_\ell$ has a neighbor in $P\cap (Y\cup \{u\})$.
Such a vertex exists as $P$ forms a connected induced subgraph of $G$.
Let $P'$ be obtained from $P$ by removing all the neighbors of $x_\ell$ in $P\cap (Y\cup\{u\})$.
Include $\{x_i\mid x_i\in P'\text{ or}\ y_i\in P'\}$ in $T$.
\item For every set $P$ in $\mathcal{P}$ containing at least one 
vertex from $Y$ and at least one vertex from $A$ but no vertices from $X$, include $\{x_i\mid y_i\in P\}$ in $T$.
\item For every set $P_Y\subseteq Y$ in $\mathcal{P}$ such that $|P_Y|\geq 2$, do the following: 
Let $x\in X$ be a vertex in $P_u$ adjacent to some vertex in $P_Y$ - such a vertex $x$
exists as otherwise $\{P_Y, P_u, P_A, P_B, P_C\}$ induces an $H$ in $G/\mathcal{P}$. Include every vertex in $P_Y$ in $T$ which are not adjacent to $x$. 
\end{enumerate}
It is sufficient to prove that, $|T|\leq k$ and for every vertex $y\in Y$, there is a vertex $x\in T$ such that $x$ is adjacent to $y$ in $G$.
It is straight-forward to verify the first part of the claim, i.e., $|T|\leq k$. 
If the second part of the claim is wrong, then there is a vertex $y_j\in Y$ such that no vertex in $T$ is adjacent to $y_j$.
Let $P_j$ be the set in $\mathcal{P}$ containing $y_j$. Based on the intersection of $P_j$ with $X,Y,A$, we have the following cases.
\begin{itemize}
    \item Assume that $P_j$ contains at least one vertex from $X$. Then by (i), either $x_j$ is in $T$ or a vertex adjacent to $y_j$ in $X$ is in $T$.
    Then we get a contradiction.
    \item Assume that $P_j$ contains at least one vertex from $A$. Then by (ii), $x_j$ is in $T$, which is a contradiction.
    \item Assume that $P_j\subseteq Y$. Then by (iii), either $x_j$ is in $T$ or a vertex adjacent to $y_j$ in $X$ is in $T$.
    Then we get a contradiction. 
\end{itemize}

Case 2: $P_u$ contains some vertices from $A$.

We claim that every set in $\mathcal{P}$ containing at least one vertex from $Y$ is equal to or adjacent to every set in $\mathcal{P}$
containing at least one vertex in $X$. For a contradiction, assume that there is a set $P_Y\in \mathcal{P}$ containing at least one vertex from $Y$
is not equal to and nonadjacent to a set $P_X\in \mathcal{P}$ containing at least one vertex from $X$. We note that $P_u$ is equal to or adjacent to $P_Y$.
Therefore, $P_X\neq P_u$. Further, $P_u$ is adjacent to $P_X$. Therefore, $P_Y\neq P_u$. Then, $\{P_Y,P_u,P_X,P_B,P_C\}$ induces an $H$, which is a contradiction.

Now we construct a set $T\subseteq X$ as follows. 
\begin{enumerate}[(a)]
\item For every set $P$ in $\mathcal{P}$ containing at least one vertex from $X$ and 
at least one vertex from $Y\cup \{u\}$, do the following: 
Let $x_\ell$ be a vertex in $P\cap X$ such that $x_\ell$ has a neighbor in $P\cap (Y\cup \{u\})$.
Such a vertex exists as $P$ forms a connected induced subgraph of $G$.
Let $P'$ be obtained from $P$ by removing all the neighbors of $x_\ell$ in $P\cap (Y\cup\{u\})$.
Include $\{x_i\mid x_i\in P'\text{ or}\ y_i\in P'\}$ in $T$.
\item For every set $P$ in $\mathcal{P}$ containing at least one 
vertex from $Y$ and at least one vertex from $A$ but no vertices from $X$, include $\{x_i\mid y_i\in P\}$ in $T$.
\item For every set $P_Y\subseteq Y$ in $\mathcal{P}$ such that $|P_Y|\geq 2$, do the following: 
Let $x\in X$ be a vertex in $T$ obtained by (a) and (b) - We note that at least one vertex is added to $T$ by (a) and (b), as otherwise 
every set $P_X$ in $\mathcal{P}$ containing at least one vertex in $X$ is a subset of $X$ and every set $P_Y$ containing at least one 
vertex in $Y$ is a subset of $Y$. 
adjacent to some vertex in $P_Y$ - such a vertex $x$
exists as otherwise $\{P_Y, P_u, P_A, P_B, P_C\}$ induces an $H$ in $G/\mathcal{P}$. 
Include every vertex in $P_Y$ in $T$ which are not adjacent to $x$. 
\end{enumerate}
\end{proof}

==> whardness/small/claw.tex <==
\subsubsection{Claw}

%\textcolor{red}{There seems an issue with this reduction. Consider the following partition $\mathcal{P}$ of vertices of $G$. 
%One set contains just $u$ and a vertex from $A$. Each of the remaining sets is a subset of $X$ or a subset of $Y$. Assume that $\mathcal{P}$
%makes $X\cup Y$ a clique. I think this is possible and it may not be possible to get a dominating set from such a partition.}

%Let $H$ be a claw. We prove that \HFC\ is $W[2]$-hard by a reduction from \DS. 

%\medskip

We give a reduction from \DS\ to \XFC{claw}. 
Let $(G',k)$ be an instance of \DS. Let $V(G')=\{ v_1, v_2, \ldots , v_n \}$. Then, $G$ is constructed as follows (refer to Figure \ref{fig: claw}):

\input{hardness/small/claw figure}

\begin{itemize}
    \item Introduce two sets of vertices $X=\{x_1, x_2, \ldots, x_n\}$, and $Y=\{y_1,y_2,\ldots,y_n\}$. Each of them forms a clique. The vertex $x_i$ is adjacent to the vertex $y_j$ if and only if $i=j$ or $v_iv_j$ is an edge in $G'$.
    \item Introduce two sets $A, B$ of $k+1$ vertices each. Further, $A\cup B$ forms a clique. In addition to this, add all possible edges between $A$ and $Y$.
    \item Introduce a vertex $u$ and make it adjacent to $X\cup A$.
\end{itemize}

\begin{lemma} \label{lem:claw-free:if}
Let $(G',k)$ be a yes-instance of \DS. Then, $(G,k)$ is a yes-instance of \XFC{claw}.
\end{lemma}

\begin{proof}
Let $T'$ be a dominating set of $G'$ such that $|T'|\leq k$. 
Let $T$ be the vertices in $X$ corresponding to the vertices in $T'$, i.e., $T=\{x_i\mid v_i\in T'\}$.
Let $\mathcal{P}$ be a partition of vertices of $G$ such that the only non-singleton set is $P=T\cup \{u\}$. It can be easily verified that
there is no vertex in $G/\mathcal{P}$ having an independent set of size 3 in its neighborhood. Therefore, $G/\mathcal{P}$
is claw-free.
\end{proof}

\begin{lemma} \label{lem_H-Free -> Dom Set}
Let $(G,k)$ be a yes-instance of {\sc $H$-Free Contraction}. Then, $(G',k)$ is a yes-instance of {\sc Dominating Set}.
\end{lemma}

\begin{proof}
Let $\mathcal{P}$ be a partition of vertices of $G$ such that $G/\mathcal{P}$ is $H$-free and \cost{\mathcal{P}} is at most $k$.
It is straight-forward to verify that there exists sets $P_A\subseteq A, P_B\subseteq B$, and $P_C\subseteq C$ in $\mathcal{P}$
such that $P_AP_BP_C$ induces a $P_3$ in $G/\mathcal{P}$.
Let $P_u$ be the set containing $u$.
We split the proof into two cases.

Case 1: $P_u$ does not contain any vertex from $A$.

If $P_u$ is not equal to and not adjacent to a set $P_Y$ containing at least one vertex from $Y$,
then $\{P_u, P_Y, P_A, P_B, P_C\}$ induces a $T_{1,2}$, which is a contradiction. 
Therefore, $P_u$ is equal to or adjacent to every set containing 
vertices from $Y$. We construct a set $T\subseteq X$ as follows. 
\begin{enumerate}[(i)]
\item For every set $P$ in $\mathcal{P}$ containing at least one vertex from $X$ and 
at least one vertex from $Y\cup \{u\}$, do the following: 
Let $x_\ell$ be a vertex in $P\cap X$ such that $x_\ell$ has a neighbor in $P\cap (Y\cup \{u\})$.
Such a vertex exists as $P$ forms a connected induced subgraph of $G$.
Let $P'$ be obtained from $P$ by removing all the neighbors of $x_\ell$ in $P\cap (Y\cup\{u\})$.
Include $\{x_i\mid x_i\in P'\text{ or}\ y_i\in P'\}$ in $T$.
\item For every set $P$ in $\mathcal{P}$ containing at least one 
vertex from $Y$ and at least one vertex from $A$ but no vertices from $X$, include $\{x_i\mid y_i\in P\}$ in $T$.
\item For every set $P_Y\subseteq Y$ in $\mathcal{P}$ such that $|P_Y|\geq 2$, do the following: 
Let $x\in X$ be a vertex in $P_u$ adjacent to some vertex in $P_Y$ - such a vertex $x$
exists as otherwise $\{P_Y, P_u, P_A, P_B, P_C\}$ induces an $H$ in $G/\mathcal{P}$. Include every vertex in $P_Y$ in $T$ which are not adjacent to $x$. 
\end{enumerate}
It is sufficient to prove that, $|T|\leq k$ and for every vertex $y\in Y$, there is a vertex $x\in T$ such that $x$ is adjacent to $y$ in $G$.
It is straight-forward to verify the first part of the claim, i.e., $|T|\leq k$. 
If the second part of the claim is wrong, then there is a vertex $y_j\in Y$ such that no vertex in $T$ is adjacent to $y_j$.
Let $P_j$ be the set in $\mathcal{P}$ containing $y_j$. Based on the intersection of $P_j$ with $X,Y,A$, we have the following cases.
\begin{itemize}
    \item Assume that $P_j$ contains at least one vertex from $X$. Then by (i), either $x_j$ is in $T$ or a vertex adjacent to $y_j$ in $X$ is in $T$.
    Then we get a contradiction.
    \item Assume that $P_j$ contains at least one vertex from $A$. Then by (ii), $x_j$ is in $T$, which is a contradiction.
    \item Assume that $P_j\subseteq Y$. Then by (iii), either $x_j$ is in $T$ or a vertex adjacent to $y_j$ in $X$ is in $T$.
    Then we get a contradiction. 
\end{itemize}

Case 2: $P_u$ contains some vertices from $A$.

We claim that every set in $\mathcal{P}$ containing at least one vertex from $Y$ is equal to or adjacent to every set in $\mathcal{P}$
containing at least one vertex in $X$. For a contradiction, assume that there is a set $P_Y\in \mathcal{P}$ containing at least one vertex from $Y$
is not equal to and nonadjacent to a set $P_X\in \mathcal{P}$ containing at least one vertex from $X$. We note that $P_u$ is equal to or adjacent to $P_Y$.
Therefore, $P_X\neq P_u$. Further, $P_u$ is adjacent to $P_X$. Therefore, $P_Y\neq P_u$. Then, $\{P_Y,P_u,P_X,P_B,P_C\}$ induces an $H$, which is a contradiction.

Now we construct a set $T\subseteq X$ as follows. 
\begin{enumerate}[(a)]
\item For every set $P$ in $\mathcal{P}$ containing at least one vertex from $X$ and 
at least one vertex from $Y\cup \{u\}$, do the following: 
Let $x_\ell$ be a vertex in $P\cap X$ such that $x_\ell$ has a neighbor in $P\cap (Y\cup \{u\})$.
Such a vertex exists as $P$ forms a connected induced subgraph of $G$.
Let $P'$ be obtained from $P$ by removing all the neighbors of $x_\ell$ in $P\cap (Y\cup\{u\})$.
Include $\{x_i\mid x_i\in P'\text{ or}\ y_i\in P'\}$ in $T$.
\item For every set $P$ in $\mathcal{P}$ containing at least one 
vertex from $Y$ and at least one vertex from $A$ but no vertices from $X$, include $\{x_i\mid y_i\in P\}$ in $T$.
\item For every set $P_Y\subseteq Y$ in $\mathcal{P}$ such that $|P_Y|\geq 2$, do the following: 
Let $x\in X$ be a vertex in $T$ obtained by (a) and (b) - We note that at least one vertex is added to $T$ by (a) and (b), as otherwise 
every set $P_X$ in $\mathcal{P}$ containing at least one vertex in $X$ is a subset of $X$ and every set $P_Y$ containing at least one 
vertex in $Y$ is a subset of $Y$. 
adjacent to some vertex in $P_Y$ - such a vertex $x$
exists as otherwise $\{P_Y, P_u, P_A, P_B, P_C\}$ induces an $H$ in $G/\mathcal{P}$. 
Include every vertex in $P_Y$ in $T$ which are not adjacent to $x$. 
\end{enumerate}


\end{proof}

Thus, putting together Lemmas \ref{lem_Dom Set -> H-Free} and \ref{lem_H-Free -> Dom Set}, we have:

\begin{theorem}
For $H \cong K_{1,3}$, {\sc $H$-Free Contraction} is $W[2]$-hard.
\end{theorem}

\begin{comment}


Let $D'$ be a dominating set, of size at most $k$, of $G'$. Let $D$ be the set of vertices in $X$ corresponding to the vertices in $D'$, i.e., 
$D = \{x_i\mid v_i\in D\}$. 

Since $(G',k)$ is a yes-instance of {\sc Dominating Set}, let $T' \subset V(G')$ such that $|T'| \leq k$ and that $T'$ is a dominating set of $G'$. Let $T=\{ y_j \in Y: v_j \in T' \}$ and $S=\{ uy: y \in T \} \subset V(G)$. We claim that $G/S$ is $H$-free.

\medskip

Toward a contradiction, let $p, q, r, s \in V(G)$ such that $\{ p,q,r,s \}$ induces a claw in $G/S$ with $p$ being the dominating vertex in the claw. Then, without loss of generality, we must have $q \in B$, $r \in X$ and $s \in T \cup \{ u \}$. As $T'$ is a dominating set of $G'$, $x_iz \in E(G/S)$ for all $z \in T \cup \{ u \}$ and $1 \leq i \leq n$. This implies that $rs \in E(G/S)$, a contradiction. Hence, $G/S$ is $H$-free.

\medskip

Moreover, $|S|=|T|=|T'| \leq k$ and hence, $S$ is a solution of $(G,k)$.


To prove that $(G',k)$ is a yes-instance of {\sc Dominating Set}, it is enough to show that for any solution $S$ of $(G,k)$ and for all $x_i \in X$, there exists a $y_j \in T_u=\{ y \in Y: uy \in S \} \cup \{ u \}$ such that $x_iy_j \in E(G)$. In this case, $T'= \{ v_j \in V(G'): y_j \in T_u \}$ is a dominating set of $G'$. Moreover, since $|T'|=|T_u|-1 \leq |S| \leq k$, $T'$ is a solution of $(G',k)$. 

\medskip

Let $S \cap E[A, \{ u \}] \neq \emptyset$, in which case, $x_iy_j \in E(G/S)$ for all $i,j$. This implies in particular that for all $x_i \in X$, there exists a $y_j \in T_u$ such that $x_iy_j \in E(G)$ and hence, we are done.

\medskip

So, let us assume that $S \cap E[A, \{  u \}] = \emptyset$. In this case, we define a new subset $S^*$ of $E(G)$ by:
\begin{enumerate}
	\item initialize $S^*=\emptyset$,
	\item for all $uy_i \in S$, let $uy_i \in S^*$,
	\item for all $z \in V(G) \setminus X$ such that $x_iz \in S$, let $uy_i \in S^*$,
	\item for all $x_ix_j \in S$ such that $uy_i \in S^*$, let $uy_j \in S^*$ and
	\item for all $y_iy_j \in S$ such that $uy_i \in S^*$, let $uy_j \in S^*$.
\end{enumerate}
We shall prove that $S^*$ is also a solution of $(G,k)$. So, toward a contradiction, let there exist $p, q, r, s \in V(G)$ such that $\{ p, q, r, s \}$ induces a claw in $G/S^*$ with $p$ being the dominating vertex of the claw. Then, without loss of generality, we must have $q \in B$, $r \in X$ and $s \in Y \cup \{ u \}$. However, as $S \cap E[A, \{ u \}] = \emptyset$, we must have $s \in T_u$. Moreover, $p=a_j \in A$ for some $j$. Now, there must exist either an $rz \in S$ or an $sz \in S$ for some $z \in V(G)$. In either case, by the construction of $S^*$ and the fact that $S \cap E[A, \{ u \}] = \emptyset$, $rs \in E(G/S^*)$, a contradiction.

\medskip

Let $T^*_u= \{ y \in Y: uy \in S^* \} \cup \{ u \}$. Then, for all $x_i \in X$, there exists a $y_j \in T^*_u$ such that $x_iy_j \in E(G)$ and hence, we are done.
\end{comment}

==> whardness/small/claw_figure.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
    
    \node at (-0.5,-0.5) {$Y$};
  \node[myv,label=above:$y_i$] (yi) at (0.5,-0.7) {};
    \node[myv,label=left:$y_j$] (yj) at (1.5,-0.3) {};
    \node at (-0.5,-3.5) {$X$};
    \node[myv,label=below:$x_i$] (xi) at (0.5,-3.5) {};
    \node[myv,label=below:$x_j$] (xj) at (1.5,-3.5) {};
    \node[myv,label=right:$a_i$] (ai) at (5.5,-0.3) {};
    \node[myv,label=above:$a_j$] (aj) at (6.5,-0.7) {};
    \node[myv,label=below:$b_i$] (bi) at (5.5,-3.5) {};
    \node[myv,label=below:$b_j$] (bj) at (6.5,-3.5) {};
    \node[myv,label=above:$u$] (u) at (3.5,-2) {};

    \draw[decorate,decoration=snake] (1,-1) -- (1,-3);

    \draw (xi) -- (xj);
    \draw (yi) -- (yj);
    %\draw (xi) -- (yj);
    \draw (yi) -- (ai);
    \draw (yi) -- (aj);
    %\draw (xj) -- (yi);
    %\draw (xj) -- (yj);
    \draw (yj) -- (ai);
    \draw (yj) -- (aj);
    \draw (xi) -- (xj);
    \draw (xi) -- (u);
    \draw (xj) -- (u);
    \draw (u) -- (ai);
    \draw (u) -- (aj);
    \draw (ai) -- (aj);
    \draw (ai) -- (bi);
    \draw (ai) -- (bj);
    \draw (aj) -- (bi);
    \draw (aj) -- (bj);
    \draw (bi) -- (bj);
    
    \node at (7.5,-0.5) {$A$};
    \node at (7.5,-3.5) {$B$};

  \draw[dashed, red] (0.0, 0.0) rectangle (2, -1);
  \draw[dashed, red] (5, 0.0) rectangle (7, -1);
  \draw[dashed, red] (0, -3) rectangle (2, -4);
  \draw[dashed, red] (5, -3) rectangle (7, -4);

    \end{tikzpicture}
    \caption{Construction of instance $(G,k)$ of {\sc Claw-Free Contraction} from the instance $(G',k)$ of {\sc Dominating Set}. The thick edges represent ``all edges".}
    \label{fig: claw}
\end{figure}

==> whardness/wstars.tex <==
\subsection{Stars}

\begin{construction}
\label{con:wstars}
Let $G'$ be a graph with a vertex set $V'=\{v_1,v_2,\ldots,v_n\}$ and let $k,t$ be integers. We construct a graph $G$ from $(G',k,t)$
as follows.
\begin{itemize}
    \item Create two cliques $X=\{x_1,x_2,\ldots,x_n\}, Y=\{y_1,y_2,\ldots,y_n\}$.
    \item Make $x_i$ adjacent to $y_j$ if and only if $i=j$ or
    $v_iv_j$ is an edge in $G'$.
    \item Create a vertex $w$ and two cliques $A$ and $B$ of $k+1$ vertices each.
    \item Make $w$ adjacent to all vertices of $X\cup A\cup B$.
    Make $A\cup B\cup Y$ a clique.
    \item Introduce $t-2$ cliques with $k+1$ vertices each and make them
    adjacent to $A$. Let the set of these vertices be denoted by $A'$.
    \item Introduce $t-2$ cliques with $k+1$ vertices each and make
    them adjacent to $B$. Let the set of these vertices be denoted by
    $B'$.
    \item Introduce $t-2$ cliques with $k+1$ vertices each and make 
    them adjacent to $X$. Let the set of these vertices be denoted by
    $X'$.
    \item Introduce a clique of $k+1$ vertices and make
    it adjacent to $Y$. Denote the set of vertices of it by $Y'$.
\end{itemize}
\end{construction}

Let $(G',k)$ be an instance of \DS. 
Let $H$ be $K_{1,t}$, for any $t\geq 4$.
We construct a graph $G$ from
$(G',k,t)$ by Construction~\ref{con:wstars}.

\begin{lemma}
\label{lem:wstars:forward}
Let $(G',k)$ be a yes-instance of \DS. Then
$(G,k)$ is a yes-instance of \XFC{H}.
\end{lemma}
\begin{proof}
Let $D$ be a dominating set of size at most $k$ of $G'$.
Let $F=\{wx_i|v_i\in D\}$. We claim that $G/F$ is $H$-free.
Let $w$ itself denote the vertex obtained by contracting all edges 
in $F$. We note that $w$ is adjacent to all vertices of $Y$
in $G/F$. We claim that the neighborhood of every vertex in $G/F$
can be covered by at most $t-1$ cliques, which proves that $G/F$
is $K_{1,t}$-free.
The neighborhood of a vertex in $A'\cup B'\cup X'\cup Y'$ can
be covered by a single clique. The neighborhood of a vertex 
in $A$ can be covered by $t-1$ cliques: $t-2$ cliques formed by $A'$
and one clique formed by $B\cup Y\cup \{w\}$.
The neighborhood of a vertex in $B$ can be covered by $t-1$ cliques:
$t-2$ cliques formed by $B'$ and one clique formed by $A\cup Y\cup \{w\}$. The neighborhood of a vertex $x$ in $X$ can be covered by $t-1$
cliques: $t-2$ cliques formed by $X'$ and one clique formed by 
$(X\cup\{w\})\setminus x$ and the neighborhood of $x$ in $Y$.
The neighborhood of a vertex $y\in Y$ can be covered by 3 cliques:
one clique each formed by $Y', B\cup\{w\}$, and the neighbors of $y$
in $X$. 
Therefore, none of the vertex in $G/F$ can be a center of a 
$K_{1,t}$ in $G/F$. This completes the proof.
\end{proof}

\begin{observation}
\label{obs:wstars}
Let $F$ be a subset of edges of $G$ such that $|F|\leq k$ and
$G/F$ is $H$-free. Then $F$ does not contain $wa, wb, xy$ for any
$a\in A, b\in B, x\in X, y\in Y$.
\end{observation}
\begin{proof}
By Observation~\ref{obs:star}, we know that if a graph contains
$K_{1,t,k+1}$, then it cannot be made $K_{1,t}$-free by at most 
$k$ edge contractions. Assume that $wa\in F$ for some $a\in A$.
Then $A'\cup B\cup X\cup \{w\}$ induces a $K_{1,t,k+1}$. 
Assume that $wb\in F$, for some $b\in B$. Then $B'\cup A\cup X\cup \{w\}$ induces a 
$K_{1,t,k+1}$. If $xy\in F$, for some $x\in X, y\in Y$, then
$Y'\cup A\cup X'\cup \{x\}$ induced $K_{1,t,k+1}$. In all
these cases, we obtain contradictions.
\end{proof}

\begin{observation}
    \label{obs:wstars:2}
    Let $\mathcal{P}$ be a partition of vertices of $G$
    such that $G/\mathcal{P}$ is $H$-free. Further assume that
    every set in $\mathcal{P}$ is either a singleton set, or a 
    subset of $X\cup \{w\}$ or a subset of $Y$. 
    Let $P_w$ denote the set in $\mathcal{P}$ containing $w$.
    Then,
    for every set $P_y\in \mathcal{P}$ such that $P_y\subseteq Y$,
    at least one vertex of $P_w\cap X$ is adjacent to at least one
    vertex of $P_y$.
\end{observation}
\begin{proof}
    For a contradiction, assume that none of the vertices in $P_y$
    is adjacent to none of the vertices of $P_w\cap X$. Then 
    there is a $K_{1,t}$ induced by $P_w, P_y$ and singleton sets
    corresponding to a vertex in $B$ and $t-2$ vertices (one from 
    each clique) corresponding to $B'$. Therefore, 
    $G/\mathcal{P}$ is not $K_{1,t}$-free, which is a contradiction.
\end{proof}
\begin{lemma}
    \label{lem:wstars:backward}
    Let $(G,k)$ be a yes-instance of \XFC{H}.
    Then $(G',k)$ is a yes-instance of \DS.
\end{lemma}
\begin{proof}
    Let $F$ be a minimal subset of edges of $G$ such that $G/F$
    is $H$-free and $|F|\leq k$.
    By Observation~\ref{obs:wstars}, the edges of type $wa,wb$, and $xy$
    cannot be in $F$. It can be easily verified that, due to the 
    limited budget, $F$ does not contain any edges of $G$ other than
    those of type $wx, xx', yy'$, for $x,x'\in X$ and $y,y'\in Y$.
    Let $\mathcal{P}$ be the partition of vertices of $G$ corresponding
    to $F$. Let $P_w$ denote the set containing $w$.
    We create a dominating set $D$ of size at most $k$ of $G'$ as
    follows.
    Include the vertices corresponding to $P_w\cap X$ in $D$, i.e., 
    include $\{v_i|x_i\in P_w\cap X\}$ in $D$. By Observation~\ref{obs:wstars:2}, for each $P_y\in \mathcal{P}$ such that $P_y\subseteq Y$, at least one vertex of $P_y$ is 
    adjacent to at least one vertex of $P_w\cap X$.
    Let $y\in P_y$ is adjacent to a vertex in $P_w\cap X$.
    Then for every vertex $y_i\in P_y\setminus \{y\}$,
    include $v_i$ in $D$. We claim that $D$ is a dominating set
    in $G'$. For a contradiction, assume that there is a vertex 
    $v_j$ not adjacent to any vertex in $D$. 
    Let $P_{y_j}\in \mathcal{P}$ be the set containing $y_j$.
    By the construction of $D$, for every vertex in $P_{y_j}$
    either $v_j$ or a vertex adjacent to $v_j$ is included in $D$.
    This gives us a contradiction. Now, it is sufficient to
    prove that \SURP$\leq k$. This follows from the fact that
    for $P_w$ we included $|P_w|-1$ vertices in $D$ and 
    for every set $P_y\in \mathcal{P}$ such that $P_y\subseteq Y$,
    we included at most $|P_y|-1$ vertices in $D$.
\end{proof}
